How Many Lines to Paint the City: Exact Edge-Cover in Temporal Graphs

Logistics and transportation networks require a large amount of resources to realize necessary connections between locations and minimizing these resources is a vital aspect of planning research. Since such networks have dynamic connections that are only available at specific times, intricate models are needed to portray them accurately. In this paper, we study the problem of minimizing the number of resources needed to realize a dynamic network, using the temporal graphs model. In a temporal graph, edges appear at specific points in time. Given a temporal graph and a natural number k, we ask whether we can cover every temporal edge exactly once using at most k temporal journeys; in a temporal journey consecutive edges have to adhere to the order of time. We conduct a thorough investigation of the complexity of the problem with respect to four dimensions: (a) whether the type of the temporal journey is a walk, a trail, or a path; (b) whether the chronological order of edges in the journey is strict or non-strict; (c) whether the temporal graph is directed or undirected; (d) whether the start and end points of each journey are given or not. We almost completely resolve the complexity of all these problems and provide dichotomies for each one of them with respect to k.

==> Proofs/poly-time-Paths_restricted-Underlying.tex <==
\subsection{Polynomial Time Algorithms for Restricted Underlying Graphs \textcolor{red}{--to be moved}}
\michelle{ToDo: Move into discusssion and long version}
    Bidirected tree we can do with paths (and probably also walks trails)
    \begin{lemma}
        \TPEECwithK{k}{(N)S-} for \textbf{directed} temporal graphs with underlying bidirected tree can be solved in $\mathcal{O}(m\log m)$.
    \end{lemma}
    DAGS, we can do with all three journey types -- strict and non-strict.
    \begin{lemma}
        \TPEECwithK{k}{(N)S-}, \TTEECwithK{k}{(N)S-} and \TWEECwithK{k}{(N)S-} for \textbf{directed} temporal graphs with underlying static DAG can be solved in $\mathcal{O}(m\log m)$.
    \end{lemma}
    Perform a ``temporal matching'' on each vertex -- on DAGS no way back; on directed undirected trees locally exactly one way back, which we can forbid.
    \michelle{Put the DAG result into the simple observations in the Prelims? Maybe also add: }
    \begin{proposition}
        Given an EEC of size $k$ on a DAG with some backwards edges. Deciding whether we can achieve $k$-EEC or need $k+1$-EEC when we input another arbitrary backwards edge, is NP-hard Even on simple temporal graphs (every edge has at most one time label).\\
        This is because otherwise, we can solve the \sat{3} formula of the para-NP-hardness result by putting in the clause-backwards-edges one by one.
    \end{proposition}
    Something that still needs to be checked:
    \begin{proposition}
        \TTEECwithK{k}{(N)S-} for \textbf{undirected} temporal graphs with an underlying undirected static tree can be solved in $\mathcal{O}(m\log m)$.
    \end{proposition}

==> Proofs/proof_fixed-terminals_UD__N_S.tex <==
\ifshort
\begin{proof}[Proof sketch]
\fi
\iflong
\begin{proof}
\fi
    % We will assume that the start- and end-terminals are each given as special vertices. Observe that a vertex can be multiple terminals, since multiple walks can start and end at the same vertex.
    % Since the time label adjacent to a vertex are unique, we can conclude for each start-terminal the unique edge adjacent to the vertex with which the walk has to start -- it is the edge with the unique smallest time label\georg{No, another walk may enter via that edge and leave immediately}.
    % Similarly, for each end-terminal we can derive the unique edge with which the walk has to end -- the edge with the unique largest time label adjacent to the vertex.
    % % A vertex may have multiple start- and end-terminals connected to it.
    % \georg{this is not how I had meant it. I specifically want to extract terminals into separate vertices, so we can argue about "normal" vertices without having to think about terminals. Like this:
    % \includegraphics[width=0.4\textwidth]{Figures/UD_TWD_representation_of_terminals.png} If multiple walks should start on a vertex, you'd have multiple of those dongles; except each of them needs a different time label because we want a strict order for the gadget constuction.}
    % In the following, we exclude terminals whenever we mention vertices.

    % First, we transform the terminals into separate vertices. % and ensure some conditions necessary for a walk eec.
    Given a temporal graph \gcal and a set of terminals, we construct a mixed static multigraph $\mathcal{S}$ with directed and undirected multiedges, and the same terminal sets. The construction will ensure that there is a temporal walk eec in \gcal if and only if there is a static walk eec in \scal. The claim then follows from \Cref{thm:static-walk-fxd-term}, which states that a static walk eec with fixed terminals can be computed in polynomial time.
    % On \scal, we then compute a static eec with fixed terminals. If such a static solution exists, we derive a walk eec in \gcal from it.

    \paragraph{Terminals.}    % Note that a vertex in \gcal can be a start and end of multiple walks while at the terminal-vertices in $\gcal'$ there will be exactly one walk starting or ending.
    For each start- and end-terminal at vertex $v$, we add an additional vertex with a single edge to $v$ with a 
    % Instead of a certain number of walks starting or ending at a vertex, we introduce additional terminal-vertices: % in addition to the existing vertices.
    % For each walk that would start on vertex $v$, we add a vertex with a single edge to $v$.
    % These edges have a 
    unique time label that is smaller, respectively larger, than all labels in \gcal.
    All other time labels are increased accordingly.
    % In turn, for each walk that would end at a vertex $v$, we add a vertex with an edge to $v$ using a unique time label greater than all existing labels.
    Note that a vertex in \gcal can be a start and end of multiple walks, while at the constructed terminals there is exactly one walk starting or ending.
    From now, the term ``vertices" will refer specifically to non-terminal vertices.

    % \iflong We observe that the temporal degree of all vertices must be even, since a walk passing through a vertex takes two edges. Otherwise we can directly reject the instance.
    % We further assume that each connected component of $\gcal$ contains at least one start and end-terminal, else the instance can be rejected as well. %\quickquestion{I think we should assume all graphs we consider to be weakly connected. Any exact edge-cover would consists of disjoint EECs for each connected component anyways.}
    % \fi

    % Now we describe how to construct a static multigraph \scal with directed and undirected edges in which any static walk eec implies a temporal walk eec in \gcal, and vice versa.

    \bigparagraph{Construction.} % of \scal}
%    Let $\gcal=\tuple{(V,E),\ecal}$ be an undirected temporal graph.
    For each vertex $v$, we create a $v$-gadget simulating the connections of $v$ at the each time step.
    Let $T(v)$ denote the multiset of labels on edges incident to $v$.
    For each time step $t\in T(v)$, create a vertex $v_t$.
    We say these vertices are placed from \emph{left to right} by increasing time label. %, meaning a vertex $v_t$ is to the \emph{left} of vertex $v_{t'}$ if and only if $t < t'$.
    Now, we connect each $v_t$ with its right neighbor $v_{t+1}$ to simulate the maximum amount of walks going through $v$ time $t$:
    % via a specific number of undirected and directed multiedges as follows:
    Let $\tdegree_{\leq t}(v)$ and $\tdegree_{\geq t+1}(v)$ be the number of temporal edges incident to $v$ with time label $\leq t$ and $\geq t+1$, respectively. The maximum amount of walks passing through has to enter before $t$ and leave after $t+1$.
    Thus, we create $\min(\tdegree_{\leq t}(v), \tdegree_{\geq t+1}(v))$ edges between $v_t$ and $v_{t+1}$. To allow some of these walks to enter before $t$ and also exit before $t$, half of these edges rounded up are directed from $v_t$ to $v_{t+1}$, while the others are undirected. A directed-undirected edge pair can then form a cycle attachable to any walk at $v_t$. 

    For each edge $(\{v, u\}, t)$ in \gcal, we add $\{v_t, u_t\}$ to \scal, and
    % \begin{figure}[h]
    %     \centering
    %     \includegraphics[width=\columnwidth]{Figures/AAAI_Walks_fixdTerm_small-figure_short.pdf}
    %     \caption{Illustration of the mixed multiedges between $v_3$, $v_4$ and $v_5$. The orange edges go to other, adjacent vertices.}
    %     \label{fig:fxd-walks_example_small}
    % \end{figure}
    for each terminal in \gcal connected to vertex $v$, we add a terminal in \scal with an edge to $v_0$.
    See \Cref{fig:UD_NS_TWD_temporal_to_static} for an illustration.

    \begin{figure*}[ht]
        \centering
        % \includegraphics[width=\textwidth]{Figures/UD_TWD_temporal_to_static_big_example.png}
        % \includegraphics[width=0.6\textwidth]{Figures/fxdWalks.pdf}
        \includegraphics[width=0.9\textwidth]{Figures/AAAI_fxdWalks.pdf}
        \caption{Illustration of how a temporal graph $\gcal$ (left) is translated into a static graph \scal (right) for \Cref{thm:UD_NS_TWD_fixed_terminals}, with start-terminals $V_S=\{s_1, s_2\}$ and end-terminals $V_E=\{e_1, e_2\}$. Vertices are replaced with gadgets based on their temporal degree.} 
        \label{fig:UD_NS_TWD_temporal_to_static}
    \end{figure*}
    %\todo{In \gcal I'm drawing the two temporal edges between v and b as different edges, which I find more intuitive, but is of course not how it's usually done. I'm fine with either} \todo{it should be easy to distinguish directed and undirected edges so the reader can see the pattern in the big gadget more easily (though colorcoding may not be the most elegant way to do it), maybe you have some IPE-tricks for this :)}

    % \bigparagraph{($\Rightarrow$)\quad}% \TWEEC in \gcal to \SWEC in \scal.}
    \paragraph{Temporal eec in \gcal to static eec in \scal.}
    % Let $\mathcal{W}$ be a walk \eecShort for \gcal. The walks in $\mathcal{W}$ can be directly translated into walks forming a static eec:
    For every temporal walk $W$, we construct a static walk with the same terminals: %start- and end-terminal:
    If $W$ sequentially traverses the edges $(\{a, v\}, t)$ and $(\{v, b\}, t')$, the corresponding static walk enters $v$-gadget via $\{a_{t},v_{t}\}$, travels $v_{t}\rightsquigarrow v_{t'}$ using directed edges (or undirected, if no directed edges remain), and exits $v$-gadget via $\{v_{t'},b_{t'}\}$.
    Observe that there is a sufficient amount of edges between neighbouring vertices $v_{t}$ and $v_{t+1}$ so that every walk crossing these vertices can use a different edge.
    % Note that at most $\tdegree_{\leq t}$ (sub-)walks may enter at $v_{t}$ or to the left of it, hence at most this many walks can go from $v_{t}$ to its right neighbor. The same constraint is placed by $\tdegree_{\geq t+1}$.
    % Hence the $\min(\tdegree_{\leq t}(v), \tdegree_{\geq t+1}(v))$ edges we created between $v_{t}$ and $v_{t+1}$ are sufficient.

    After translating the temporal walks into static walks this way, some edges between some $v_t$ and its right neighbor $v_{t+1}$ may remain unused. We show that this number is always even and the edges can be attached to existing walks:
    The number of edges between $v_t$ and $v_{t+1}$ equals the maximum walks possibly present in $v$ right at time $t$, which is achieved when every undirected edge before $t$ is directed towards $v$.
    If there is one less walk present, then this walk had to enter at $\{a_i,v_i\}$ and exit at $\{v_j,b_j\}$, both before $t$.
    Therefore, the walk which would have entered at $\{v_j,b_j\}$ is also missing.
    Since directed edges are used before undirected edges, at least half of the remaining edges are undirected.
    These edges form a cycle going back and forth between $v_{t}$ and $v_{t+1}$, which can be inserted into any walk visiting $v_{t}$.
    % The argument is equivalent for $\tdegree_{\geq t+1}(v) \leq \tdegree_{\leq t}(v)$ by considering edges at or to the right of $t_{t+1}$.
    % After translating the temporal walks this way, some edges within a gadget may remain unused. Thus number is always even. The number of edges between $v_t$ and $v_{t+1}$ corresponds to the maximum number of walks possibly present in $v$ right after time $t$. To reach this maximum, every undirected edge before $t$ has to be directed into $v$. If there is one less walk present, then this walk had to enter at $\{a_i,v_i\}$ and exit at $\{v_j,b_j\}$ before $t$. Therefore, there is also the walk missing which would have entered at $\{v_j,b_j\}$.
    % After translating the temporal walks this way, some edges within a gadget may remain unused. We first show that the number of unused edges between a vertex $v_{t}$ and its right neighbor is even. W.l.o.g., let $\tdegree_{\leq t}(v) \leq \tdegree_{\geq t+1}(v)$ and let $x$ be the number of walks that exit the gadget via an edge to the left of (or at) $v_{t}$. Each of these walks also has to enter the gadget via an edge to the left of (or at) $v_{t}$, since by construction walks only move through gadgets from left to right. In turn, there are $\tdegree_{\leq t}(v)-2x$ other walks entering to the left of (or at) $v_{t}$, and those walks each take an edge from $v_{t}$ to its right neighbor. Given that there are $\tdegree_{\leq t}(v)$ such edges, $\tdegree_{\leq t}(v) - (\tdegree_{\leq t}(v) - 2x)=2x$ edges will remain unused, which is an even number. \george{reverse the argument\georg{I'm not sure how :/}}
    % This even number of unused edges can be inserted into existing walks:
    % Recall that directed edges are used before undirected edges. In particular, if $\tdegree_{\leq t}(v)$ is odd, at least one directed edge will be used. Therefore, of the $2x$ remaining edges, at least half of them are undirected.
    % These edges form a cycle going back and forth between $v_{t}$ and its right neighbor, which can be inserted into any walk visiting $v_{t}$. The argument is equivalent for $\tdegree_{\geq t+1}(v) \leq \tdegree_{\leq t}(v)$ by considering edges at or to the right of $t_{t+1}$.

    % In the end, we are left with a set of walks starting at start terminals and ending at end terminals that use each edge exactly once. This is a static walk exact edge-cover for \scal. \george{This paragraph only for long version}\georg{seems like an abrupt end to me then; also this proof sketch will only exist in the short version}

    % \bigparagraph{($\Leftarrow$)\quad}% \SWEC in \scal to \TWEEC in \gcal.}
    \bigparagraph{Static eec in \scal to temporal eec in \gcal.}
    A static eec in \scal cannot be directly translated into a temporal eec in \gcal.
    For a temporal eec, each walk must exit a vertex via a time label greater than the one by which it entered the vertex.
    In \scal, this corresponds to every walk exiting a gadget to the right of its entry point, which is not guaranteed due to the undirected edges. Refer to \Cref{fig:UD_TWD_redirected_static_walks} (top) for an illustration of a walk violating this property.
    However, we can modify any static eec on \scal to be time-respecting.
    The general idea is that any walk going ``back in time'' has to overlap with at least one walk with which it can swap suffixes. Refer to \Cref{fig:UD_TWD_redirected_static_walks} (bottom) for an illustration of such a swap, working as follows:

    Let $W_1$ enter at $v_{t_j}$ and exit at $v_{t_i}$ with $t_i < t_j$.
    Then it used an undirected edge $\{v_{t_{i+1}},v_{t_{i}}\}$.
    By construction, there is at least one directed edge $(v_{t_i},v_{t_{i+1}})$ taken by some walk $W_2$ that entered to the left of $v_{t_i}$ and exits to the right. Otherwise, by the parity argument for the edges, at least one edge between $v_{t_{i}}$ and $v_{t_{i+1}}$ would not be covered.
    We now swap the suffixes of $W_1$ and $W_2$ and therefore reduce the number of backwards taken edges by at least one. This is continued until no edges are taken backwards.
    % See \Cref{fig:UD_TWD_redirected_static_walks} for an illustration. 
    \begin{figure}[ht]
        \centering
        % \includegraphics[width=0.8\textwidth]{Figures/UD_TWD_redirected_static_walks.png}
        \includegraphics[width=\columnwidth]{Figures/short-version-fxdWalks-suffixswitch_smaller.pdf}
        \caption{Suffix-switch between two walks $W_1$ and $W_2$.
        }
        \label{fig:UD_TWD_redirected_static_walks}
    \end{figure}
    % After performing this procedure for every walk, we have a static \eecShort for which every walk exits a gadget to the right of where it enters.\george{slightly informal}
    
    Finally, we can translate the time-respecting static eec into a temporal eec by contracting the gadgets back into vertices.


% \georg{TODO: figure out the run time. With $n$ vertices and $m$ edges in \gcal, I think \scal has $\mathcal{O}(n \cdot \tmax)$ vertices and $\mathcal{O}(m+n\cdot \tmax^2)$ edges. And plug that into the runtime of the static algo. Though I don't think it's actually that bad. If I remember correctly, the static algo is a flow, which would use capacities instead of multiedges. Then it would be more like $m+ n \cdot \tmax$ edges.}
    % \georg{If a min-cost flow with negative edge cost works here (also on undirected graphs) it can replace this paragraph.}
    % \georg{actually \Cref{lem:static_walks_fixed_terminals} can maybe solve this after the directed edges are abstracted away. How convenient. Someone confirm pls}
    % To solve \SWEC on an undirected graph with fixed terminals, we run a flow algorithm:
    % Every start-terminal becomes a source producing one flow unit, and every end-terminal becomes a sink consuming one unit.
    % Edges have a capacity of $1$.
    % Now find a maximum flow.
    % If the flow is able to satisfy all sources and sinks, it yields a set of initial walks from every start-terminal to a different end-terminal.
    % There may be edges with unused capacity remaining.
    % However, all vertices in our construction have an even degree, which stays true after removing all edges used in these initial walks.
    % Thus the remaining edges form a collection of cycles, which can be repeatedly integrated into the existing walks.
\end{proof}
    

